The weak order on integer posets

We explore lattice structures on integer binary relations (i.e. binary relations on the set $\{1, 2, \dots, n\}$ for a fixed integer $n$) and on integer posets (i.e. partial orders on the set $\{1, 2, \dots, n\}$ for a fixed integer $n$). We first observe that the weak order on the symmetric group naturally extends to a lattice structure on all integer binary relations. We then show that the subposet of this weak order induced by integer posets defines as well a lattice. We finally study the subposets of this weak order induced by specific families of integer posets corresponding to the elements, the intervals, and the faces of the permutahedron, the associahedron, and some recent generalizations of those.

==> figures/counterexample_trans.tex <==

\begin{tabular}{c|c|c|c|c}
$\rel \in \ITrans(3)$ &
$\rel[S] \in \ITrans(3)$ &
$\rel \meetR \rel[S] \notin \ITrans(3)$ &
$\tc{\left(\rel \meetR \rel[S]\right)} \nleq \rel, \rel[S]$ &
$\rel \meetT \rel[S] \in \ITrans(3)$
\\
\scalebox{0.5}{\input{relations/poset312.tex}} &
\scalebox{0.5}{\input{relations/poset231.tex}} &
\scalebox{0.5}{\input{relations/R2.tex}} &
\scalebox{0.5}{\input{relations/Full3.tex}} &
\scalebox{0.5}{\input{relations/poset123.tex}}
\end{tabular}

==> figures/interval_2143_4231.tex <==
% Explicit interval [2143, 4231]

\begin{tikzpicture}
\node(T4231) at (0,0) {$\sigma' = 4231$};
\node(T2431) at (-1,-1) {$2431$};
\node(T4312) at (1,-1) {$4312$};
\node(T2413) at (0,-2) {$2413$};
\node(T2143) at (0,-3) {$\sigma = 2143$};
\draw (T4231) -- (T2431);
\draw (T4231) -- (T4312);
\draw (T2431) -- (T2413);
\draw (T4312) -- (T2413);
\draw (T2413) -- (T2143);
\end{tikzpicture}

==> figures/relations/Empty3.tex <==
% Empty relation of size 3

\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (2,0) {3};
\draw[->,line width = 0.5, color=white, opacity=0] (T1) edge [bend left=70] (T3);
\draw[->,line width = 0.5, color=white, opacity=0] (T3) edge [bend left=70] (T1);
\end{tikzpicture}
